"Chasing Shadows": Understanding Personal Data Externalization and Self-Tracking for Neurodivergent Individuals

We examine how neurodivergent individuals experience creating, interacting with, and reflecting on personal data about masking. Although self-tracking is often framed as enabling self-insight, this is rarely our experience as neurodivergent individuals and researchers. To better understand this disconnect, we conducted a two-phase qualitative study. First, a workshop where six participants with autism and/or ADHD crafted visual representations of masking experiences. Then, three participants continued by designing and using personalized self-tracking focused on unmasking over two weeks. Using reflexive thematic analysis of activities and interviews, we find that self-tracking imposes substantial interpretive and emotional demands, shaped by context-dependencies that challenge assumptions in self-tracking. We also find that facilitated sharing of experiences might validate emotional responses and support reflection. We identify three emotional dimensions that shape engagement with personal data in a working model of emotion in self-tracking, and discuss implications for designing self-tracking and reflective practices that incorporate peer support and better account for context and emotional labor.

==> tables/selftrackingapproaches.tex <==
\begin{table*}
  \caption{Self-tracking approaches designed and implemented by participants in Phase II.}
  \label{tab:selftrackingapproaches}
 \begin{sffamily}
  \begin{tabular}{l p{3.8cm} p{3.8cm} p{3.8cm}}
\toprule
    & \textbf{P3} & \textbf{P5} & \textbf{P6} \\
\midrule
  \textbf{Goal} & Test hypothesis: masking less around neurodivergent friends & Capture emotional complexity and identify patterns in masking behaviors & Recognize when masking occurs; build sustainable routine \\
  & & & \\
  \textbf{Method} & Activity-based logs with predefined questions (free text + Likert scales) & Pre-constructed diagram with 64 items (emotions, thoughts, needs) marked when relevant & Mark ``X'' on existing work schedule when masking noticed; add optional reflections \\
  & & & \\
  \textbf{Context} & Social situations and activities & School (during class hours) & Work (weekdays only) \\
  & & & \\
  \textbf{Frequency} & Per social event/activity & Hourly while at school & Daily (with occasional gaps) \\
  & & & \\
  \textbf{Duration} & 1 week (14 reports) & 1 week (34 reports) & 2 weeks (5 reports) \\
\bottomrule
  \end{tabular}
 \end{sffamily}
\end{table*}
